Superfast Configuration-Space Convex Set Computation on GPUs for Online Motion Planning

In this work, we leverage GPUs to construct probabilistically collision-free convex sets in robot configuration space on the fly. This extends the use of modern motion planning algorithms that leverage such representations to changing environments. These planners rapidly and reliably optimize high-quality trajectories, without the burden of challenging nonconvex collision-avoidance constraints. We present an algorithm that inflates collision-free piecewise linear paths into sequences of convex sets (SCS) that are probabilistically collision-free using massive parallelism. We then integrate this algorithm into a motion planning pipeline, which leverages dynamic roadmaps to rapidly find one or multiple collision-free paths, and inflates them. We then optimize the trajectory through the probabilistically collision-free sets, simultaneously using the candidate trajectory to detect and remove collisions from the sets. We demonstrate the efficacy of our approach on a simulation benchmark and a KUKA iiwa 7 robot manipulator with perception in the loop. On our benchmark, our approach runs 17.1 times faster and yields a 27.9% increase in reliability over the nonlinear trajectory optimization baseline, while still producing high-quality motion plans.

==> sections/drm.tex <==
\section{Generating Collision-Free Polygonal Paths using Dynamic Roadmaps}\label{sec:drm}

\rccomment{Since DRM implementation isn't the focus of this paper, I think a lot of this could be moved to a background section, and parts of it could be moved to the following section ``Motion Planning Pipeline'' in a subsection before ``Finding a Target Configuration'' (maybe a subsection called ``Computing a Single Path'' before ``Inflating a Single Path''). I think the offline construction details could also be placed in an Appendix. I can do this later when I do a more detailed pass.}
In this paper, we employ dynamic roadmaps (DRM) to rapidly find collision-free piecewise-linear paths for our robots, between a start configuration and a goal specified as an end-effector pose. DRMs, introduced in \cite{leven2002framework}, approximate $\Cfree$ with a probabilistic roadmap (PRM) \cite{kavraki1996probabilistic}, discretize the robot workspace into voxels, and build large lookup tables that map activated voxels to nodes and edges of the PRM that are in collision. The key idea is that pruning the PRM given a set of activated voxels is faster and leads to better motion plans than running a single query motion planner \cite{kallman2004motion} given the current perceived environment. Hence, DRMs enable us to offload parts of the computational burden of motion planning to the offline construction of the roadmap, which, in our examples, required on the order of $10^{12}$ collision checks.

In our pipeline, we closely follow the implementation in \cite{cheng2023motion} that can leverage our GPU-accelerated collision checker to build large-scale DRMs. Similarly, we skip constructing the edge collision map, see \cite{liu2006path}, and use lazy collision checking online to invalidate colliding edges \cite{bohlin2000path}. In the following, we detail the employed procedure for constructing our DRMs offline, and how we rapidly find polygonal paths online given perception using our constructed roadmaps.

\subsection{Offline Roadmap Construction}\label{ssec:offlinedrm}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/DRM_collision_set.png}
    \caption{DRM indicating  offline voxels in yellow, showing 3 out of 232 configs that collide with the center offline voxel. Voxel radius (yellow sphere )is ~5cm, $n_x = 25,n_y = 34,n_z = 26 $}
    \label{fig:enter-label}
\end{figure}

Our offline construction of the DRM closely follows \cite{cheng2023motion}. First, we sample a batch of configurations uniformly in the collision-free configuration space of our system. Next, we construct a PRM that only adds edges between two configurations if both their $L_2$ distance in configuration space is smaller than $d_\text{CS}$ and the distance in task space of a selected frame is less than $d_\text{TS}$. We further limit the number of outgoing connections to other nodes by $k$ for each node during construction. In a final step, we ensure that the adjacency matrix is symmetric by adding missing edges.

In a next step, we discretize the taskspace of the robot into voxels, and check each node of the roadmap for collisions against every voxel. We use a sphere with radius $\tfrac{\sqrt{3}}{2}s$, where $s$ is the side length of a voxel, that circumscibes each voxel for collision checking. 

Finally, we collect the results in 4 data structures: 1. A node map $\calM_n: \calI\rightarrow\calC$ that maps a node identification number (node id) $i\in\calI$ to its configuration, 2. a node adjacency map $\calM_a: \calI\rightarrow\calP(\calI)$, where $\calP$ denotes the power set of $\calI$, which maps a node id to all its neighbors, 3. a collision map $\calM_c: \calJ \rightarrow \calP(I)$ that maps a voxel identification number (voxel id) $j\in\calJ$ to all node ids that are in collision if the voxel $j$ is active, and finally 4. a pose map $\calM_p: \calI \rightarrow SE(3)$ that maps each node id to its corresponding end-effector pose.

\subsection{Online Planning given Perception}\label{ssec:offlinedrm}
Online, we assume we are given a point cloud observation of the world, a starting configuration and a target pose $P_\text{T}\in SE(3)$. The planning then proceeds in three phases. In the first phase, we build the collision set $CS\in\calP(I)$ that contains the ids of all nodes that are colliding with the point cloud. This is done by determining all voxels containing points and subsequently using the collision map $\calM_c$ to find all nodes in collision. In the second phase, we determine a goal configuration by solving an inverse kinematics problem. In this paper, we use the pose map $\calM_p$ and the collisions set to find collision-free configurations that lie near $P_\text{T}$, where we measure the distance as a weighted sum of the translation and rotation error.
If needed, the closest configuration is used to warmstart a small IK problem to improve the solution. {\color{red} How much detail add here? the focus should be on the region generation so saving space here is probably fine?}
Finally, similarly to \cite{cheng2023motion}, we connect the start and the goal node up to the roadmap, and use $A^*$ \cite{hart1968formal} combined lazy collision checking and greedy short cutting to find our collision-free polygonal path. For all collision-checks, we down-sample the point cloud by voxelizing the points and selecting their collision geometries as spheres. Again, we chose the radius to be $\tfrac{\sqrt{3}}{2}$-times the bin size and the centers to lie at the centers of the bins. Note that for collision checking we often use a smaller size than during the offline construction of the roadmap.

{\color{red} Finish figure, reference it}



==> sections/multiple_paths.tex <==
\section{Expanding Multiple Paths}\label{sec:multi-path}
